Computational Aspects of the Calculus of Structure

Logic is the science of correct inferences and a logical system is a tool to prove assertions in a certain logic in a correct way. There are many logical systems, and many ways of formalizing them, e.g., using natural deduction or sequent calculus. Calculus of structures (CoS) is a new formalism proposed by Alessio Guglielmi in 2004 that generalizes sequent calculus in the sense that inference rules can be applied at any depth inside a formula, rather than only to the main connective. With this feature, proofs in CoS are shorter than in any other formalism supporting analytical proofs. Although it is great to have the freedom and expressiveness of CoS, under the point of view of proof search more freedom means a larger search space. And that should be restricted when looking for complete automation of deductive systems. Some efforts were made to reduce this non-determinism, but they are all basically operational approaches, and no solid theoretical result regarding the computational behaviour of CoS has been achieved so far. The main focus of this thesis is to discuss ways to propose a proof search strategy for CoS suitable to implementation. This strategy should be theoretical instead of purely operational. We introduce the concept of incoherence number of substructures inside structures and we use this concept to achieve our main result: there is an algorithm that, according to our conjecture, corresponds to a proof search strategy to every provable structure in the subsystem of FBV (the multiplicative linear logic MLL plus the rule mix) containing only pairwise distinct atoms. Our algorithm is implemented and we believe our strategy is a good starting point to exploit the computational aspects of CoS in more general systems, like BV itself.

==> abstract.tex <==
Logic is the science of correct inferences and a logical system is a tool to prove assertions in a certain logic in a correct way. There are many logical systems, and many ways of formalizing them, e.g., using natural deduction or sequent calculus. Calculus of structures (\cos) is a new formalism proposed by Alessio Guglielmi in 2004 that generalizes sequent calculus in the sense that inference rules can be applied at any depth inside a formula, rather than only to the main connective. With this feature, proofs in \cos\ are shorter than in any other formalism supporting analytical proofs. Although it is great to have the freedom and expressiveness of \cos, under the point of view of proof search more freedom means a larger search space. And that should be restricted when looking for complete automation of deductive systems. Some efforts were made to reduce this non-determinism, but they are all basically operational approaches, and no solid theoretical result regarding the computational behaviour of \cos\ has been achieved so far. The main focus of this thesis is to discuss ways to propose a proof search strategy for \cos\ suitable to implementation. This strategy should be theoretical instead of purely operational. We introduce the concept of incoherence number of substructures inside structures and we use this concept to achieve our main result: there is an algorithm that, according to our conjecture, corresponds to a proof search strategy to every provable structure in the subsystem of \FBV\ (the multiplicative linear logic \MLL\ plus the rule \mix) containing only pairwise distinct atoms. Our algorithm is implemented and we believe our strategy is a good starting point to exploit the computational aspects of \cos\ in more general systems, like \BV\ itself.

==> agradecimentos.tex <==
Agradecimentos agradecimentos agradecimentos agradecimentos agradecimentos agradecimentos agradecimentos agradecimentos agradecimentos agradecimentos agradecimentos agradecimentos agradecimentos agradecimentos agradecimentos agradecimentos agradecimentos agradecimentos.

==> bingo.tex <==
{\Large Resultados Principais}

\begin{Lemma}[\emph{Estratégia para $\incnumber{S}{a}{\dual{a}} = 0$}]
\label{lema:incnumber0}
		Seja $S$ uma estrutura demonstrável em \FBV\ com apenas pares de átomos dois a dois distintos tal que $S=S'\pars{a,\dual{a}}$. Então podemos aplicar a regra $\ruleaidown$ sobre $a$ e $\dual{a}$:
		
		$$
			\dernote{}{}{S'\pars{a,\dual{a}}}
			{\leaf{\strpr{}{}
			{S'\{ \ \}}}}
		$$
		
\end{Lemma}		

\begin{Lemma}[\emph{Estratégia para $\incnumber{S}{a}{\dual{a}} = 1$}]
\label{lema:incnumber1}
		Seja $S$ uma estrutura demonstrável em \FBV\ com apenas pares de átomos dois a dois distintos tal que $S = S'\pars{a,\aprs{\dual{a},X}}$. Então $S'\aprs{\pars{a,\dual{a}},X}$ também é demonstrável e podemos fazer:
		
		$$
			\dernote{}{}{S'\pars{a,\aprs{\dual{a},X}}}
			{\leaf{\strpr{}{}
			{S'\aprs{\pars{a,\dual{a}},X}}}}
		$$
		
\end{Lemma}	

\begin{Lemma}[Estratégia para $\incnumber{S}{a}{\dual{a}} \geq 2$]
\label{lema:incnumber2}

	Seja $S$ uma estrutura demonstrável em \FBV\ com pares de átomos dois a dois distintos. Então existem $R$, $T$, $P'$ e $P''$ tais que:
	
	$$
		\dernote{\rules}{}{\pars{\aprs{R,T},P',P''}}
		{\rootnote{\rules}{}{\pars{\aprs{\pars{T,P''},R},P'}}
		{\leaf{\strpr{}{}{\aprs{\pars{R,P'},\pars{T,P''}}{}}}}}
	$$
	
	Além disso, para todo par de átomos duais $a, \dual{a} \in \occ{S}$, $\incnumber{S}{a}{\dual{a}}$ permanece o mesmo ou diminui ao longo da aplicação das regras switch acima expostas.
	
\end{Lemma}

\begin{Theorem}[Resultado Principal]
\label{teorema:resultado-principal}
Existe um algoritmo que corresponde a uma estratégia de prova para toda estrutura provável $S$ em \FBV\ contendo apenas pares de átomos dois a dois distintos. 
\end{Theorem}
\begin{proof}
Considere a estratégia fornecida pelos lemas \ref{lema:incnumber0}, \ref{lema:incnumber1},  \ref{lema:incnumber2}. Comece a prova pela redução da subestrutura que contém ocorrências de átomos $a$ e $\dual{a}$ de número de incoerência módulo coerência igual a $0$ ou $1$ (pelos lemas \ref{lema:incnumber0} e \ref{lema:incnumber1} sei como agir em cada caso). Se não houver tal subestrutura, existem subestrturuas $R$, $T$, $P'$ e $P''$ que satisfazem o Lema \ref{lema:incnumber2} e posso reduzir o número de incoerência de alguns pares de átomos duais sem alterar a demonstrabilidade da estrutura. Posso aplicar o Lema \ref{lema:incnumber2} indefinidamente até que um par de átomos possua o número de incoerência igual a $0$ ou a $1$, casos em que já sei como proceder. Se um estágio for atingido sobre o qual não se possa avançar, é porque a estrutura já não era provável desde o início (pelos lemas \ref{lema:incnumber0}, \ref{lema:incnumber1} e \ref{lema:incnumber2}).
\end{proof}

%\begin{Definition}
%
%Seja uma estrutura da forma $\pars{\aprs{R,T},P}$, em que $P = \pars{P_{1},\hdots,P_{n}}$ e $P_{i}$ não é um par próprio, $1 \leq i \leq n$. O \emph{grafo de partição} $\grafocompleto{G}{\aprs{R,T}} = (V,E)$ relacionado a esta estrutura é definido da seguinte maneira:
%
%	\begin{description}
%		\item [Vértices:] $V = \{R\} \ \ \cup \ \ \{T\} \ \ \cup \ \ \{ \ P_{i} \ \ | \ \ 1 \leq i \leq n \ \}$
%		\item [Arestas:] $E = \{ \ (v,w) \ \ | \ \ v, w \in V \ \ e \ \ \occ{v} \cap \occ{\dual{w}} \neq \emptyset \ \}$
%	\end{description}
%
%\end{Definition}
%
%Note que a definição de $\grafocompleto{G}{\aprs{R,T}}$ depende da escolha de quem é $R$ e $T$ na estrutura. Por exemplo, para a estrutura $\pars{\aprs{a,b},\aprs{c,d}}$ poderiam-se definir os grafos $\grafocompleto{G}{\aprs{a,b}}$ e $\grafocompleto{G}{\aprs{c,d}}$. Quando não houver ambigüidade, diremos apenas $\grafo{G}$ no lugar de $\grafocompleto{G}{\aprs{R,T}}$.
%
%\newpage
%
%\begin{Notation}
%
%Em um grafo $\grafocompleto{G}{\aprs{R,T}} = (V,E)$, usamos:
%	
%		$$
%			\xymatrix{
%				\vertice{P_{i}}{x_{1},x_{2},x_{3},\hdots}
%			}
%		$$
%	
%		para representar um vértice $v$ do grafo $G$, onde $P_{i}$ é a estrutura que compõe o vértice e $x_{1}, x_{2}, x_{3}, \hdots$ são uma ou algumas (mas não necessariamente todas) ocorrências de átomos de $P_{i}$
%
%\end{Notation}
%
%\newpage
%
%\begin{Lemma}
%	\label{lema:caminhoRT}
%	Seja $\pars{\aprs{R,T},P}$ uma estrutura demonstrável em \FBV\ com pares de átomos dois a dois distintos. Então o grafo $\grafocompleto{G}{\aprs{R,T}}$ não possui um caminho do vértice $R$ até o vértice $T$.
%	
%	\begin{proof}
%			
%		Pelo teorema de \emph{Shallow Splitting}, se $\pars{\aprs{R,T},P}$ é demonstrável em \FBV, então:
%		
%		$$ 
%			\vcenter{\strpr{}{}{\pars{\aprs{R,T},P}}}  		
%			\ \ \ \ \ equivale \ a \ \ \ \ \ 		
%			\vcenter{\strder{\Pi_{1}}{}{P}{\leaf{\pars{P',P''}}}}
%			\ \ \ \ \ e \ \ \ \ \		
%			\vcenter{\strpr{\Pi_{2}}{}{\pars{R,P'}}}		 
%			\ \ \ \ \ e \ \ \ \ \		
%			\vcenter{\strpr{\Pi_{3}}{}{\pars{T,P''}}}		
%		$$
%		
%		A derivação $\Pi_{2}$ nos diz que $\pars{R,P'}$ é demonstrável. Como estamos lidando apenas com estruturas com pares de átomos dois a dois distintos, segue diretamente que para todo $a \in \occ{\pars{R,P'}}$ seu dual $\dual{a} \in \occ{\pars{R,P'}}$. Raciocínio análogo vale sobre a derivação $\Pi_{3}$. 
%		
%		Temos, então, que após a aplicação da derivação $\Pi_{1}$ sobre uma estrutura demonstrável $\pars{\aprs{R,T},P}$, obtemos uma nova estrutura demonstrável $\pars{\aprs{R,T},P',P''}$ da seguinte forma:
%		
%	$$
%		\strder{\Pi_{1}}{}{\pars{\aprs{R,T},P}}{\leaf{\pars{\aprs{R,T},P',P''}}}
%	$$ 
%	
%	Além disso, as seguintes condições são válidas:
%	
%	\begin{description}
%		\item[C1] $\forall a \in \occ{\pars{R,P'}}, \dual{a} \in \occ{\pars{R,P'}}$
%		\item[C2] $\forall b \in \occ{\pars{T,P''}}, \dual{b} \in \occ{\pars{T,P''}}$
%	\end{description}
%	
%	
%	Vamos analisar a estrutura $\pars{\aprs{R,T},P',P''}$ cujo grafo é $\grafocompleto{G'}{\aprs{R,T}}$. Suponha que haja na estrutura $R$ uma ocorrência de átomo $x$, cujo dual $\dual{x}$ esteja em uma estrutura $P_{j}$. Então $\grafocompleto{G'}{\aprs{R,T}}$ possui um subgrafo da forma:
%	
%	$$
%		\xymatrix{
%			\vertice{R}{x} \ar@{-}[r] & \vertice{P_{j}}{\dual{x}}
%		}
%	$$
%	
%	A estrutura $P_{j}$ deve estar em $P'$, para satisfazer a condição \textbf{C1}. Suponha que haja uma ocorrência atômica $y$ em $P_{j}$ cujo dual $\dual{y}$ esteja em outra estrutura $P_{j}'$. Então $\grafocompleto{G'}{\aprs{R,T}}$ possui um subrafo da forma:
%	
%	$$
%		\xymatrix{
%			\vertice{R}{x} \ar@{-}[r] & \vertice{P_{j}}{\dual{x},y} \ar@{-}[r] & \vertice{P_{j}'}{\dual{y}}
%		}
%	$$
%	
%	Também, pela condição \textbf{C1}, a subestrutura $P_{j}'$ deve estar em $P'$. Por transitividade, podemos dizer que todo vértice $P_{j}$ que esteja ligado por um caminho ao vértice $R$ deve fazer parte de $P'$. 
%	
%	De maneira análoga, podemos concluir que a condição \textbf{C2} implica que todo vértice $P_{j}$ que esteja ligado por um caminho ao vértice $T$ deve fazer parte de $P''$. 
%	
%	Suponha, então, que haja um caminho de $R$ até $T$ em $\grafocompleto{G'}{\aprs{R,T}}$. Nesse caso, existe um $P_{j}$ que está ligado tanto a $R$ quanto a $T$ e que, portanto, deveria fazer parte ao mesmo tempo de $P'$ e $P''$, o que não é possível. Logo em $\pars{\aprs{R,T},P',P''}$ o grafo $\grafocompleto{G'}{\aprs{R,T}}$ não possui um caminho entre $R$ e $T$.
%	
%	Falta apenas mostrar que, se de $\pars{\aprs{R,T},P',P''}$ (cujo grafo é $\grafocompleto{G'}{\aprs{R,T}}$) podemos obter em \FBV\ uma estrutura $\pars{\aprs{R,T},P}$ (cujo grafo é $\grafocompleto{G}{\aprs{R,T}}$) via uma derivação $\Pi$ (figura abaixo), então se $\grafocompleto{G'}{\aprs{R,T}}$ não possui caminho entre $R$ e $T$, $\grafocompleto{G}{\aprs{R,T}}$ também não o possui.
%	
%	$$
%		\strder{\Pi}{}{\pars{\aprs{R,T},P}}{\leaf{\pars{\aprs{R,T},P',P''}}}
%	$$
%	
%	Vamos mostrar o contrapositivo desta afirmação: se $\grafocompleto{G}{\aprs{R,T}}$ possui um caminho entre $R$ e $T$, então $\grafocompleto{G'}{\aprs{R,T}}$ também possui. Se $\grafocompleto{G}{\aprs{R,T}}$ possui um caminho entre $R$ e $T$, $\grafocompleto{G}{\aprs{R,T}}$ possui um subgrafo da forma:
%	
%	$$
%		\xymatrix{
%			\vertice{P_{r}}{x} \ar@{-}[r] & \vertice{P_{j}}{\dual{x},y} \ar@{-}[r] & \vertice{P_{t}}{\dual{y}}
%		}
%	$$
%	
%	onde existe um caminho de $P_{r}$ até $R$ e um caminho de $P_{t}$ até $T$. 
%	
%	Teríamos que desfazer de alguma forma o caminho que liga $R$ a $T$ passando por $P_{j}$, obtendo algo do tipo:
%	
%	$$
%		\xymatrix{
%			\verticesimples{P_{r}}{} & \vertice{P_{x}}{x} \ar@{-}[l] & \vertice{P_{y}}{y} \ar@{-}[r] \ar@{-}[r] & \verticesimples{P_{t}}{}
%		}
%	$$ 
%	
%	Ou seja, teríamos que ter uma derivação $\Pi$ do tipo:
%	
%	$$
%		\strder{\Pi}{}{S\{P_{j}\{x,y\}\}}{\leaf{S'\{P_{x}\{x\},P_{y}\{y\}\}}}
%	$$
%	
%	A única maneira que temos de fazer isto é aplicando regras de inferência sobre as subestruturas $P_{i}$ de $P$. Note que teríamos que separar duas ocorrências de átomos $x$ e $y$ que pertenciam a uma mesma estrutura copar de forma que agora $x$ pertença a uma estrutura copar e $y$ a outra. A regra $\ruleaidown$ não contribui para isto, pois ela só pode ser aplicada internamente a cada estrutura $P_{i}$. Só resta a regra switch. Mas a regra switch é da forma:
%	
%	$$
%		\dernote{\rules}{}{\pars{\aprs{X,Y},Z}}{\leaf{\aprs{\pars{X,Z},Y}}}
%	$$
%	
%	e, de baixo para cima, ela somente aumenta o tamanho de uma estrutura copar, ou seja, se $x$ e $y$ pertencem a uma mesma estrutura copar, não tem como separá-los. Logo não é possível desfazer o caminho entre $R$ e $T$ e, necessariamente, $\grafocompleto{G}{\aprs{R,T}}$ possui um caminho entre $R$ e $T$.
%	
%	\end{proof}
%	
%\end{Lemma}
%
%\newpage
%
%\begin{Theorem}
%\label{teorema:particaoP}
%	
%	Seja $S = \pars{\aprs{R,T},P}$ uma estrutura demonstrável em \FBV\ com pares de átomos dois a dois distintos. Consideremos $P = \pars{P_{1}, P_{2}, \hdots, P_{n}}$, onde $P_{i}$ não é uma estrutura par própria e $1 \leq i \leq n$.
%	
%	Sejam $P'$ e $P''$ estruturas que satisfaçam o Teorema de \emph{Shallow Splitting}:
%	
%	$$ 
%		\vcenter{\strpr{}{}{\pars{\aprs{R,T},P}}}  		
%		\ \ \ \ \ equivale \ a \ \ \ \ \ 		
%		\vcenter{\strder{\Pi_{1}}{}{P}{\leaf{\pars{P',P''}}}}
%		\ \ \ \ \ e \ \ \ \ \		
%		\vcenter{\strpr{\Pi_{2}}{}{\pars{R,P'}}}		 
%		\ \ \ \ \ e \ \ \ \ \		
%		\vcenter{\strpr{\Pi_{3}}{}{\pars{T,P''}}}		
%	$$
%	
%	Então existe uma ordenação das subestruturas $P_{i}$ dentro de $P$ tal que $P' = \pars{P_{1},\hdots,P_{k}}$ e $P'' = \pars{P_{k+1},\hdots,P_{n}}$, onde $1 \leq k \leq n$. Em outras palavras, existe uma maneira de construir a derivação $\Pi_{1}$ utilizando somente regras triviais (relação de equivalência sintática $=$).
%	
%	\begin{proof}
%	
%		Vamos provar por indução no tamanho da derivação $\Pi_{1}$. Seja $\rho$ a última regra de inferência aplicada sobre $P$:
%		
%		$$
%			\dernote{\rho}{}{P}{\leaf{W}}
%		$$
%		
%		\begin{description}
%		
%			\item[Caso base:]
%				\ \\
%				$\rho$ é a própria relação de equivalência:
%				
%				$$
%					\dernote{=}{}{P}{\leaf{\pars{P',P''}}}
%				$$
%			
%			\item[Casos indutivos:]
%				\ \\
%				\begin{enumerate}
%				
%					\item $\rho = \ruleaidown$ ou  $\rho = \rules$ e o redex está em $P'$:
%					
%					
%						$$ 
%							\vcenter{\dernote{\rho}{}{\pars{P',P''}}{\leaf{\strder{}{}{\pars{P'_{*},P''}}{\leaf{\pars{P',P''}}}}}}
%							\ \ \ \ \ e \ \ \ \ \		
%							\vcenter{\strpr{\Pi_{2}}{}{\pars{R,P'}}}		 
%							\ \ \ \ \ e \ \ \ \ \		
%							\vcenter{\strpr{\Pi_{3}}{}{\pars{T,P''}}}		
%						$$
%						
%						equivalem a
%					
%						$$
%							\vcenter{\dernote{=}{}{\pars{P',P''}}{\leaf{\strder{}{}{\pars{P',P''}}{\leaf{\pars{P',P''}}}}}}
%							\ \ \ \ \ e \ \ \ \ \		
%							\vcenter{\dernote{\rho}{}{\pars{R,P'}}{\leaf{\strpr{\Pi_{2}'}{}{\pars{R,P'_{*}}}}}}
%							\ \ \ \ \ e \ \ \ \ \		
%							\vcenter{\strpr{\Pi_{3}}{}{\pars{T,P''}}}
%						$$
%					
%						e aplicamos a hipótese de indução.
%						
%					\item $\rho = \ruleaidown$ ou  $\rho = \rules$ e o redex está em $P''$: 
%					\ \\
%					Análogo ao caso anterior.
%																
%					\item $\rho = \rules$ e o redex envolve $P'$ e $P''$:
%					
%						$$
%							\dernote{\rules}{}{P\pars{\aprs{P_{1}',P_{2}'},P''}}{\leaf{P\aprs{\pars{P_{1}',P''},P_{2}'}}}
%						$$
%					
%						Divide-se em casos:
%					
%						\begin{enumerate}
%							
%							\item O grafo $\grafocompleto{G}{\aprs{R,T}}$ do redex era tal que:
%							
%								$$
%									\xymatrix{
%										\verticesimples{P_{r}} \ar@{-}[r] & \verticesimples{\aprs{P_{1}',P_{2}'}} & \verticesimples{P''} \ar@{-}[r] & \verticesimples{P_{t}}
%									}
%								$$
%								
%								onde existe um caminho de $P_{r}$ até $R$ e um caminho de $P_{t}$ até $T$.
%								
%								Após a aplicação da regra de inferência o grafo $\grafocompleto{G'}{\aprs{R,T}}$ do contractum passa a ter um subgrafo da forma:
%								
%								$$
%									\xymatrix{
%										\verticesimples{P_{r}} \ar@{-}[r] & \verticesimples{P\aprs{\pars{P_{1}',P''},P_{2}'}} \ar@{-}[r] & \verticesimples{P_{t}}
%									}
%								$$
%								
%								e passamos a ter um caminho entre $R$ e $T$, o que torna a estrutura não demonstrável, pelo lema \ref{lema:caminhoRT}.
%							 
%							\item O grafo $\grafocompleto{G}{\aprs{R,T}}$ do redex era tal que:
%							
%								$$
%									\xymatrix{
%										\verticesimples{\aprs{P_{1}',P_{2}'}} & \verticesimples{P''} \ar@{-}[r] & \verticesimples{P_{t}}
%									}
%								$$
%								
%								ou seja, não existe um caminho de $\aprs{P_{1}',P_{2}'}$ a $R$ nem a $T$ . Basta fazer com que $\aprs{P_{1}',P_{2}'}$ (juntamente com o grafo induzido pelos vértices adjacentes) seja movido para $P''$, de forma que possamos considerar que o redex encontrava-se todo dentro de $P''$ desde o princípio. Aplica-se então a hipótese de indução.
%
%						\end{enumerate}
%					
%				\end{enumerate}
%			
%		\end{description}
%	
%	\end{proof}
%	
%
%\end{Theorem}
%
%\begin{Theorem}
%\label{}
%	Seja uma estrutura $S$ demonstrável em \FBV\ com pares de átomos dois a dois distintos. $S$ não é da forma:
%	
%	$$ S\pars{ \ \ S_{1}\aprs{A_{1}\{a_{1}\},A_{2}'\{\dual{a}_{2}\}} \ \ , \ \ S_{2}\aprs{A_{2}\{a_{2}\},A_{3}'\{\dual{a}_{3}\}} \ \ , \ \hdots \ \ , \ \	
%S_{n}\aprs{A_{n}\{a_{n}\},A_{1}'\{\dual{a}_{1}\}} \ \ } $$
%	
%	Ou seja, a teia de interação de $S$ não possui uma subteia da forma:
%	
%	$$
%		\xymatrix{
%			a_{1} \ar@{~}[dr] & a_{2} \ar@{~}[dr] & \hdots \ar@{~}[dr] & a_{n-1} \ar@{~}[dr] & a_{n} \ar@{~}[dllll] \\
%			\dual{a}_{1} & \dual{a}_{2} & \hdots & \dual{a}_{n-1} & \dual{a}_{n}
%		}
%	$$
%	
%	onde a as relações $a_{i} \downarrow a_{j}$, que deveriam ser representadas por $\xymatrix{a_{i} \ar@{-}[r] & a_{j}}$, foram omitidas.
%	
%	\begin{proof}
%		
%		Escolhemos o contexto $S_{j}\{ \ \}$ de menor tamanho. Vamos demonstrar por indução no tamanho do contexto $S_{j}\{\ \}$, ou seja, indução sobre $|S_{j}\{ \ \}|$
%		
%		\begin{description}
%		
%			\item[Caso base:]
%			\ \\
%			$|S_{j}\{ \ \}| = 0$. Nesse caso $S_{j}\{ \circ \} = \circ$ e temos que:
%			
%			$S = \pars{\aprs{A_{j}\{a_{j}\},A_{j+1}\{a_{j+1}\}},P}$
%			
%			Vamos fazer $R = A_{j}\{a_{j}\}$ e $T = A_{j+1}\{a_{j+1}\}$. Agora vamos verificar o grafo $\grafocompleto{G}{\aprs{R,T}}$:
%			
%			$$
%				\xymatrix{
%					& & \vertice{S_{1}}{a_{1},\dual{a}_{2}} \ar@{-}[d] & \\
%					& & \hdots \ar@{-}[d] & \\
%					& & \vertice{S_{j-2}}{a_{j-2},\dual{a}_{j-1}} \ar@{-}[d] & \\
%					& & \vertice{S_{j-1}}{a_{j-1},\dual{a}_{j}} & \\
%					\vertice{R}{a_{j}} \ar@{-}[rru] &   & & & \vertice{T}{a_{j+1}} \ar@{-}[dll] \\
%					& & \vertice{S_{j+1}}{a_{j+1},\dual{a}_{j+2}} \ar@{-}[d] & \\
%					& & \vertice{S_{j+2}}{a_{j+2},\dual{a}_{j+3}} \ar@{-}[d] & \\
%					& & \hdots \ar@{-}[d] & \\
%					& & \vertice{S_{n}}{a_{n},\dual{a}_{1}} \ar@/_6pc/ [uuuuuuuu] & \\
%				}
%			$$
%			
%			Notamos que há um caminho $R, S_{j-1}, S_{j-2}, \hdots, S_{1}, S_{n}, S_{n-1}, S_{j+2}, S_{j+1}, T$ entre $R$ e $T$ em $\grafocompleto{G}{\aprs{R,T}}$. Pelo lema \ref{lema:caminhoRT} a estrutura $S$ não é provável.
%		
%			\item[Casos indutivos:]
%			\ \\
%			$|S_{j}\{ \circ \}| > 0$. Nesse caso $S_{j}\{ \circ \} \neq \circ$ e podemos reescrever $S$ como:
%			
%			Se $S = S'_{j}\aprs{A_{j}\{a_{j}\},A_{j+1}\{a_{j+1}\}\}}$ fosse provável, então poderíamos aplicar o teorema de \emph{Context Reduction} sobre $S$ e obter:
%			
%			\begin{enumerate}
%			
%				\item $S'_{j} = \pars{S'\{ \ \},P}$, $P \neq \circ$ e $S'\{ \ \}$ não é um par próprio.
%				
%					\begin{enumerate}
%						
%						\item $S'\{\circ\} = \circ$
%							\ \\
%							Nesse caso temos $S = \pars{\aprs{A_{j}\{a_{j}\},A_{j+1}\{a_{j+1}\}\}},P'}$, que equivale ao caso base.
%							
%						\item $S'\{ \ \} = \aprs{S''\{ \ \}, P'}$
%							\ \\
%							Nesse caso $S = \pars{\aprs{S''\aprs{A_{j}\{a_{j}\},A_{j+1}\{a_{j+1}\}},P'},P}$
%							Mas, se $S$ fosse provável, pelo teorema de \emph{Shallow Splitting} teríamos:
%							
%							$$ 
%								\vcenter{\strpr{}{}{\pars{\aprs{S''\aprs{A_{j}\{a_{j}\},A_{j+1}\{a_{j+1}\}},P'},P}}}  		
%								\ \ \ \ \ equivale \ a \ \ \ \ \ 	
%							$$
%							$$	
%								\vcenter{\strder{\Pi_{1}}{}{P}{\leaf{\pars{P_{1},P_{2}}}}}
%								\ \ \ \ \ e \ \ \ \ \		
%								\vcenter{\strpr{\Pi_{2}}{}{\pars{S''\aprs{A_{j}\{a_{j}\},A_{j+1}\{a_{j+1}\}},P_{1}}}}		 
%								\ \ \ \ \ e \ \ \ \ \		
%								\vcenter{\strpr{\Pi_{3}}{}{\pars{T,P_{2}}}}		
%							$$
%							
%							Então podemos construir:
%							
%							$$
%								\strder{\Pi_{1}}{}{\pars{\aprs{S''\aprs{A_{j}\{a_{j}\},A_{j+1}\{a_{j+1}\}},P'},P}}
%								{\rootnote{\rules}{}{\pars{\aprs{S''\aprs{A_{j}\{a_{j}\},A_{j+1}\{a_{j+1}\}},P'},P_{1},P_{2}}}
%								{\leaf{\strder{\Pi_{3}}{}{\pars{\aprs{\pars{P',P_{2}},S''\aprs{A_{j}\{a_{j}\},A_{j+1}\{a_{j+1}\}}},P_{1}}}
%								{\leaf{\pars{S''\aprs{A_{j}\{a_{j}\},A_{j+1}\{a_{j+1}\}},P_{1}}}}}}}
%							$$
%							
%							e em seguida usar a hipótese de indução, pois $|S''\{\ \}| < |S'_{j}\{\ \}|$.
%					\end{enumerate}
%				
%				\item $S'_{j}\{ \ \} = \aprs{S'\{ \ \}, P}$, $P \neq \circ$
%					\ \\
%					Este caso não se aplica, pela forma de $S$.
%			
%			\end{enumerate}
%		
%		\end{description}
%		
%	\end{proof}
%	
%\end{Theorem}
%
%\begin{Corollary}
%
%É condição necessária para uma estrutura $S$ ser demonstrável em \FBV\ com pares de átomos dois a dois distintos que $S$ não possua uma subteia de interação da forma:
%
%	$$
%		\xymatrix{
%			a_{1} \ar@{~}[dr] & a_{2} \ar@{~}[dr] & \hdots \ar@{~}[dr] & a_{n-1} \ar@{~}[dr] & a_{n} \ar@{~}[dllll] \\
%			\dual{a}_{1} & \dual{a}_{2} & \hdots & \dual{a}_{n-1} & \dual{a}_{n}
%		}
%	$$
%	
%	onde a as relações $a_{i} \downarrow a_{j}$, que deveriam ser representadas por $\xymatrix{a_{i} \ar@{-}[r] & a_{j}}$, foram omitidas.
%	
%\end{Corollary}
%
%\newpage
%
%\begin{Lemma}[Estratégia para $\incnumber{S}{a}{\dual{a}}$ > 1]
%\label{lema:incnumber2}
%
%Seja $S = \pars{\aprs{R,T},P}$ uma estrutura demonstrável em \FBV\ com pares de átomos dois a dois distintos. Então é possível fazer:
%
%	$$
%		\dernote{=}{}{\pars{\aprs{R,T},P}}
%		{\rootnote{s}{}{\pars{\aprs{R,T},P_{1},P_{2}}}
%		{\root{s}{\pars{\aprs{\pars{T,P_{2}},R},P_{1}}}		
%		{\leaf{\strpr{}{}{\aprs{\pars{R,P_{1}},\pars{T,P_{2}}}}}}}}
%	$$
%	
%	\begin{proof}
%	
%		Pelo teorema de \emph{Shallow Splitting}, se $\pars{\aprs{R,T},P}$ é demonstrável em \FBV então:
%		
%		$$ 
%			\vcenter{\strpr{}{}{\pars{\aprs{R,T},P}}}  		
%			\ \ \ \ \ equivale \ a \ \ \ \ \ 		
%			\vcenter{\strder{\Pi_{1}}{}{P}{\leaf{\pars{P_{1},P_{2}}}}}
%			\ \ \ \ \ e \ \ \ \ \		
%			\vcenter{\strpr{\Pi_{2}}{}{\pars{R,P_{1}}}}		 
%			\ \ \ \ \ e \ \ \ \ \		
%			\vcenter{\strpr{\Pi_{3}}{}{\pars{T,P_{2}}}}		
%		$$
%	
%		Mas pelo teorema \ref{teorema:particaoP}, a derivação $\Pi_{1}$ pode ser construída utilizando apenas regras de equivalência sintática $=$:
%		
%		$$ 
%			\vcenter{\strpr{}{}{\pars{\aprs{R,T},P}}}  		
%			\ \ \ \ \ equivale \ a \ \ \ \ \ 		
%			\vcenter{\dernote{=}{}{P}{\leaf{\pars{P_{1}',P_{2}'}}}}
%			\ \ \ \ \ e \ \ \ \ \		
%			\vcenter{\strpr{\Pi_{2}'}{}{\pars{R,P_{1}'}}}		 
%			\ \ \ \ \ e \ \ \ \ \		
%			\vcenter{\strpr{\Pi_{3}'}{}{\pars{T,P_{2}'}}}		
%		$$
%		
%		E então podemos montar a derivação desejada:
%		
%		$$
%			\dernote{=}{}{\pars{\aprs{R,T},P}}
%			{\rootnote{s}{}{\pars{\aprs{R,T},P_{1}',P_{2}'}}
%			{\root{s}{\pars{\aprs{\pars{T,P_{2}'},R},P_{1}'}}		
%			{\leaf{\strder{\Pi_{2}'}{}{\aprs{\pars{R,P_{1}'},\pars{T,P_{2}'}}}
%			{\leaf{\strpr{\Pi_{3}'}{}{\aprs{T,P_{2}'}}}}}}}}
%		$$
%	
%	\end{proof}
%
%\end{Lemma}

%\begin{Theorem}
%
%	Seja $S = \pars{\aprs{R,T},P}$ uma estrutura demonstrável em \FBV\ com pares de átomos dois a dois distintos. Consideremos $P = \pars{P_{1}, P_{2}, \hdots, P_{n}}$, onde $P_{i}$ não é uma estrutura par própria e $1 \leq i \leq n$.
%	
%	Sejam $P'$ e $P''$ estruturas que satisfaçam o Teorema de \emph{Shallow Splitting}:
%	
%	$$ 
%		\vcenter{\strpr{}{}{\pars{\aprs{R,T},P}}}  		
%		\ \ \ \ \ equivale \ a \ \ \ \ \ 		
%		\vcenter{\strder{\Pi_{1}}{}{P}{\leaf{\pars{P',P''}}}}
%		\ \ \ \ \ e \ \ \ \ \		
%		\vcenter{\strpr{\Pi_{2}}{}{\pars{R,P'}}}		 
%		\ \ \ \ \ e \ \ \ \ \		
%		\vcenter{\strpr{\Pi_{3}}{}{\pars{T,P''}}}		
%	$$
%	
%	Então existe uma ordenação das subestruturas $P_{i}$ dentro de $P$ tal que $P' = \pars{P_{1},\hdots,P_{k}}$ e $P'' = \pars{P_{k+1},\hdots,P_{n}}$, onde $1 \leq k \leq n$.
%	
%\begin{Remark}
%		Note que o teorema equivale a dizer que a derivação $\Pi_{1}$ possui somente regras triviais (relação de equivalência sintática $=$). Portanto, encontrar a derivaçaõ $\Pi_{1}$ é o mesmo que simplesmente separar a estrutura par $P$ em duas estruturas pares menores $P'$ e $P''$.
%\end{Remark}
%	
%\begin{proof}
%
%	Vamos modelar o problema de encontrar a ordenação das subestruturas $P_{i}$ na estrutura maior $P$ como um problema de grafos. Seja o grafo não direcionado $G = (V,E)$ tal que: 
%	
%	\begin{description}
%		\item [Vértices:] $V = \{R\} \ \ \cup \ \ \{T\} \ \ \cup \ \ \{ \ P_{i} \ \ | \ \ 1 \leq i \leq n \ \}$
%		\item [Arestas:] $E = \{ \ (v,w) \ \ | \ \ v, w \in V \ \ e \ \ \occ{v} \cap \occ{\dual{w}} \neq \emptyset \ \}$
%	\end{description}
%	
%	Se conseguirmos particionar os vértices deste grafo (com excessão dos vértices $R$ e $T$) em dois conjuntos de vértices $\Upsilon'$ e $\Upsilon''$ equivalendo, respectivamente, às estruturas $P'$ e $P''$ que satisfazem o teorema de \emph{Shallow Splitting}, então claramente temos a prova que procuramos: basta chamar os elementos do conjunto de $\Upsilon'$ de $P_{1}, \hdots, P_{k}$ e fazer $P' = \pars{P_{1}, \hdots, P_{k}}$ e os elementos do conjunto $\Upsilon''$ de $P_{k+1}, \hdots, P_{n}$ e fazer $P'' = \pars{P_{k+1}, \hdots, P_{n}}$.
%	
%	Para encontrar esta partição do grafo $G$, vamos atentar para alguns pontos importantes. Primeiramente, a derivação $\Pi_{2}$ do teorema de \emph{Shallow Splitting} nos diz que $\pars{R,P'}$ é demonstrável. Portanto, sabemos que para todo $a \in \occ{\pars{R,P'}}$ seu dual $\dual{a} \in \occ{\pars{R,P'}}$. Como a estrutura oringial $S$ só possui pares de átomos dois a dois distintos, uma conseqüência direta é que toda ocorrência de átomo $a$ em $R$ não pode ter uma ocorrência dual $\dual{a}$ em $P''$, ou seja, $\occ{P''} \cap \occ{\dual{R}} = \emptyset$. Por raciocínio análogo sobre a prova $\Pi_{3}$, concluímos que $\occ{P'} \cap \occ{\dual{T}} = \emptyset$. 
%	
%	Assim, temos as seguintes \emph{condições de particionamento de $P$}:
%	
%	\begin{description}
%		\item[C1] $\forall a \in \occ{\pars{R,P'}}, \dual{a} \in \occ{\pars{R,P'}}$
%		\item[C2] $\forall b \in \occ{\pars{T,P''}}, \dual{b} \in \occ{\pars{T,P''}}$
%		\item[C3] $\occ{P''} \cap \occ{\dual{R}} = \emptyset$
%		\item[C4] $\occ{P'} \cap \occ{\dual{T}} = \emptyset$
%	\end{description}
%	
%	Vamos analisar um exemplo. Em primeiro lugar, vamos definir a notação:
%	
%	$$
%		\xymatrix{
%			\vertice{P_{i}}{x_{1},x_{2},x_{3},\hdots}
%		}
%	$$
%	
%	para representar um vértice $v$ do grafo $G$, onde $P_{i}$ é a estrutura que compõe o vértice e $x_{1}, x_{2}, x_{3}, \hdots$ são uma ou algumas (mas não necessariamente todas) ocorrências de átomos de $P_{i}$.
%	
%	 Suponha que haja na estrutura $R$ uma ocorrência de átomo $x$, cujo dual $\dual{x}$ esteja em uma estrutura $P_{j}$. Então $G$ possui um subgrafo da forma:
%	
%	$$
%		\xymatrix{
%			\vertice{R}{x} \ar@{-}[r] & \vertice{P_{j}}{\dual{x}}
%		}
%	$$
%	
%	A estrutura $P_{j}$ deve ser incluída na partição $P'$, para satisfazer a condição de particionamento \textbf{C1}. Suponha que haja uma ocorrência atômica $y$ em $P_{j}$ cujo dual $\dual{y}$ esteja em outra estrutura $P_{j}'$. Então $G$ possui um subrafo da forma:
%	
%	$$
%		\xymatrix{
%			\vertice{R}{x} \ar@{-}[r] & \vertice{P_{j}}{\dual{x},y} \ar@{-}[r] & \vertice{P_{j}'}{\dual{y}}
%		}
%	$$
%	
%	Também, pela condição \textbf{C1}, a subestrutura $P_{j}'$ deve ser incluída em $\Upsilon'$. Podemos generalizar e dizer que todo vértice $P_{j}$ que esteja ligado por um caminho ao vértice $R$ deve ser acrescentado ao conjunto $\Upsilon'$. 
%	
%	Da mesma forma, pela condição \textbf{C2}, todo vértice $P_{j}$ que esteja ligado por um caminho ao vértice $T$ deve ser acrescentado ao conjunto $\Upsilon''$. 
%	
%	Além disso, as condições \textbf{C3} e \textbf{C4} dizem que um vértice não pode ser adicionado, ao mesmo tempo, ao conjunto $\Upsilon'$ e $\Upsilon''$. Graficamente, as condições de particionamento dizem que em $G$ não pode haver um caminho do vértice $R$ até o vértice $T$, ou seja, a seguinte situação não é permitida:
%	
%	$$
%		\xymatrix{
%			\verticesimples{R}{} \ar@{-}[r] & \verticesimples{P_{j}'}{} \ar@{-}[r] & \hdots & \verticesimples{P_{j}''}{} \ar@{-}[l] &  \verticesimples{T}{} \ar@{-}[l]
%		}
%	$$
%	
%	Em outras palavras, o conjunto $\Upsilon'$ deve conter o componente conectado de $G$ que contém o vértice $R$, enquanto o conjunto $\Upsilon''$ deve conter o componente conectado de $G$ que contém o vértice $T$. Vamos chamar de $G'$ e $G''$ os componentes conectados que contêm, respectivamente, o vértice $R$ e o vértice $T$. Se o grafo $G$ possuir um outro componente $G'''$ (conectado ou não) que não esteja conectado a $G'$ nem a $G''$, então o componente $G'''$ pode ser adicionado ao conjunto $\Upsilon'$ ou ao conjunto $\Upsilon''$ sem prejuízo das condições de particionamento. 
%	
%	Podemos resumir da seguinte forma: se uma estrutura $S = \pars{\aprs{R,T},P}$ é provável em \FBV\ com pares de átomos dois a dois distintos, então deve necessariamente haver uma maneira de transformar $P$ de tal forma que o grafo gerado $G$ possua componentes desconectadas entre si $G'$ e $G''$ tal que $G'$ contém o vértice $R$ e $G''$ contém o vértice $T$. 
%	
%	Se a estrutura $S = \pars{\aprs{R,T},P}$ já possui um grafo $G$ satisfazendo a condição acima, basta aplicar o seguinte algoritmo para encontrar o particionamento desejado:
%	
%	\begin{description}
%		
%		\item[Passo 1:] Faça $\Upsilon = \Upsilon' = \emptyset$ e $\Psi = \{ \ P_{i} \ \ | \ \ 1 \leq i \leq n \ \}$.
%		
%		\item[Passo 2:] Para todo $P_{i} \in V \ \ | \ \ (P_{i}, R) \in E$, faça $\Upsilon' = \Upsilon' \cup \{P_{i}\}$ e $\Psi = \Psi \backslash \{P_{i}\}$.
%		
%		\item[Passo 3:] Para todo $P_{j} \in \Upsilon' \ \ | \ \ (P_{j}, P_{i}) \in E$, faça $\Upsilon' = \Upsilon' \cup \{P_{i}\}$ e $\Psi = \Psi \backslash \{P_{i}\}$.
%		
%		\item[Passo 4:] Se, ainda há algum $P_{j} \in \Upsilon', P_{i} \in \Psi \ \ | \ \ (P_{i},P_{j}) \in E $, volte ao Passo 3. Senão, se $T$ foi incluído em $\Upsilon'$, ocorreu erro. Pare.
%		
%		\item[Passo 5:] Para todo $P_{i} \in V \ \ | \ \ (P_{i}, T) \in E$, faça $\Upsilon'' = \Upsilon'' \cup \{P_{i}\}$ e $\Psi = \Psi \backslash \{P_{i}\}$.
%		
%		\item[Passo 6:] Para todo $P_{j} \in \Upsilon'' \ \ | \ \ (P_{j}, P_{i}) \in E$, faça $\Upsilon'' = \Upsilon'' \cup \{P_{i}\}$ e $\Psi = \Psi \backslash \{P_{i}\}$.
%		
%		\item[Passo 7:] Se, ainda há algum $P_{j} \in \Upsilon'', P_{i} \in \Psi \ \ | \ \ (P_{i},P_{j}) \in E $, volte ao Passo 6.
%		
%		\item[Passo 8:] Se $\Psi \neq \emptyset$, faça $\Upsilon' = \Upsilon' \cup \Psi$ e $\Psi = \emptyset$.
%		
%		\item[Passo 9:] Para finalizar, faça $P'$ ser um par que contém todos os elementos de $\Upsilon'$, ou seja, se $\Upsilon' = \{ P_{1}, \hdots, P_{k} \}$, então $P' = \pars{P_{1}, \hdots, P_{k}}$. Da mesma forma, se $\Upsilon'' = \{ P_{k+1}, \hdots, P_{n} \}$, então $P'' = \pars{P_{k+1}, \hdots, P_{n}}$.
%		
%	\end{description}
%		
%	O algoritmo funciona se o grafo $G$ possuir componentes $G'$ e $G''$ desconectados entre si tais que $R$ pertence a $G'$ e $T$ pertence a $G''$. Só falta mostrar que $G$ \emph{sempre} possui as componentes $G'$ e $G''$.
%	
%	Suponha que $G$ não possua as componentes $G'$ e $G''$, então $G$ possui um subgrafo da forma:
%	
%	$$
%		\xymatrix{
%			\verticesimples{P_{r}}{} & \vertice{P_{j}}{x,y} \ar@{-}[l] \ar@{-}[r] & \verticesimples{P_{t}}{}
%		}
%	$$ 
%	
%	em que existe um caminho de $P_{r}$ até o vértice $R$ e de $P_{t}$ até o vértice $T$. Para que consigamos uma partição de $G$ em duas, temos que desfazer de alguma forma o caminho que liga $R$ a $T$ passando por $P_{j}$, obtendo algo do tipo:
%	
%	$$
%		\xymatrix{
%			\verticesimples{P_{r}}{} & \vertice{P_{x}}{x} \ar@{-}[l] & \vertice{P_{y}}{y} \ar@{-}[r] \ar@{-}[r] & \verticesimples{P_{t}}{}
%		}
%	$$ 
%	
%	Ou seja, teríamos que ter uma derivação $\Pi$ do tipo:
%	
%	$$
%		\strder{\Pi}{}{S\{P_{j}\{x,y\}\}}{\leaf{S'\{P_{x}\{x\},P_{y}\{y\}\}}}
%	$$
%	
%	A única maneira que temos de fazer isto é aplicando regras de inferência sobre as subestruturas de $P$. Note que teríamos que separar duas ocorrências de átomos $x$ e $y$ que pertenciam a uma mesma estrutura copar de forma que agora $x$ pertença a uma estrutura copar e $y$ a outra. A regra $\ruleaidown$ não contribui para isto, pois ela só pode ser aplicada internamente a cada estrutura $P_{i}$. Só resta a regra switch. Mas a regra switch é da forma:
%	
%	$$
%		\dernote{\rules}{}{\pars{\aprs{X,Y},Z}}{\leaf{\aprs{\pars{X,Z},Y}}}
%	$$
%	
%	e, de baixo para cima, ela somente aumenta o tamanho de uma estrutura copar, ou seja, se $x$ e $y$ pertencem a uma mesma estrutura copar, não tem como separá-los. Se não é possível separá-los, então não é possível separar o grafo $G$ em componentes, e a estrutura $\pars{\aprs{R,T},P}$ não seria provável, o que contradiz a nossa premissa.
%	
%\end{proof}
%
%\end{Theorem}


==> dedicatoria.tex <==
Dedicatória dedicatória dedicatória dedicatória dedicatória dedicatória dedicatória dedicatória dedicatória dedicatória dedicatória dedicatória dedicatória dedicatória dedicatória dedicatória dedicatória dedicatória dedicatória dedicatória dedicatória dedicatória dedicatória dedicatória.

==> incnumber2.tex <==
\begin{Lemma}[Estratégia para $\incnumber{S}{a}{\dual{a}} > 1$]
\label{lema:incnumber2}
Seja $S$ uma estrutura provável em \FBV\ com átomos dois a dois distintos tal que $\incnumber{S}{a}{\dual{a}}>1$ para todo $a\in \occ{S}$. Seja $a\in \occ{S}$ o átomo com menor número de incoerência módulo coerência na estrutura.
				Então temos um dos seguintes casos para $S\{a,\dual{a}\}$:
				
				\ \\				
				\begin{tabular}{lll}
				
					1 & $S'\pars{a,\aprs{T\{\dual{a}\},Y}}$ \\
					
					2 & $S'\pars{\aprs{R\{a\},X},\aprs{T\{\dual{a}\}},Y}$ \\
					
				\end{tabular}
				
				\ \\				
				O caso 2 se divide em três subcasos:
				
				\ \\				
				\begin{tabular}{lll}
					
					2a & $R\{\circ\} = T\{\circ\} = \circ$: & $S\{a,\dual{a}\} = S'\pars{\aprs{a,X},\aprs{\dual{a},Y}}$\\
								
					2b & $R\{\circ\} = \circ$ e $T\{\circ\} \neq \circ$: & $S\{a,\dual{a}\}= S'\pars{\aprs{a,X},\aprs{T\{\dual{a}\},Y}}$\\
								
					2c & $R\{\circ\} \neq \circ$ e $T\{\circ\} \neq \circ$: & $S\{a,\dual{a}\}= S'\pars{\aprs{R\{a\},X},\aprs{T\{\dual{a}\},Y}}$\\
				\end{tabular}
				
				\ \\
				, onde $X,Y \neq \circ$				
				
				\ \\				
				Além disso:
								
				\ \\
				\begin{tabular}{llll}
					1  & Se temos $S'\pars{a,\aprs{T\{\dual{a}\},Y}}$ & $\implies$ & podemos fazer $\vcenter{\dernote{\rules}{}{S'\pars{a,\aprs{T\{\dual{a}\},Y}}}{\leaf{S'\aprs{\pars{a,T\{\dual{a}\}},Y}}}}$ \\
										
					2a & Se temos $S'\pars{\aprs{a,X},\aprs{\dual{a},Y}}$ & $\implies$ & $\vcenter{\dernote {\rules }{}{S\pars{\aprs{a,X},\aprs{\dual{a},Y}}} {
	  \rootnote{\rules
	  }{}{S\aprs{\pars{a,{\aprs{\dual{a},Y}}},X}}
	  {\root{\ruleaidown}{S\aprs{\pars{a,\dual{a}},Y,X}}
	  {\leaf{S\aprs{Y,X}}}}}}$ \\
					
					2b & Se temos $S'\pars{\aprs{a,X},\aprs{T\{\dual{a}\},Y}}$ & $\implies$ & \\
					
					2c & Se temos $S'\pars{\aprs{R\{a\},X},\aprs{T\{\dual{a}\},Y}}$ & $\implies$ & 				$S'\aprs{\pars{T\{\dual{a}\},\aprs{R\{a\},X}},Y}$ ou \\
					  &                                                              &        &
					  $S'\aprs{\pars{R\{a\},\aprs{T\{\dual{a}\},Y}},X}$ é provável. \\
				\end{tabular}
				
\begin{proof}

	A primeira parte da prova segue facilmente da definição de número de incoerência e da minimalidade de $a$.

Seja $S\{a,\dual{a}\}=\pars{X\{a\},Y\{\dual{a}\}}$. A prova da provabilidade é por indução sobre o número de incoerência de $\{a, \dual{a}\}$.

\begin{itemize}
\item Caso 1: \ \ $S'\pars{\aprs{a,X},\aprs{\dual{a},Y}}$

	$(\Rightarrow)$ Por indução no tamanho da derivação $\Pi$ de $S\pars{\aprs{a,X},\aprs{\dual{a},Y}}$. Se $\occ{X} \ \cap \ \occ{Y} \ = \ \emptyset$, então obviamente não será criada nenhuma inconsistência. Se $\occ{X} \ \cap \ \occ{Y} \ \neq \ \emptyset$, a estrutura inicial conteria uma subestrutura equivalente a $\pars{\aprs{a,b},\aprs{\dual{a},\dual{b}}}$, que sabemos não ser provável pela condição $C_{2}$ do Teorema~\ref{teorema:condicoes}.

$(\Leftarrow)$ Considere a prova
	$$
	\dernote {\rules }{}{S\pars{\aprs{a,X},\aprs{\dual{a},Y}}} {
	  \rootnote{\rules
	  }{}{S\aprs{\pars{a,{\aprs{\dual{a},Y}}},X}}
	  {\root{\ruleaidown}{S\aprs{\pars{a,\dual{a}},Y,X}}
	  {\leaf{S\aprs{Y,X}}}}}
	$$

\item Caso 2: \ \ $S'\pars{\aprs{a,X},\aprs{T\{\dual{a}\},Y}}$, \  \ $T\{\circ\} \neq \circ$

	Considere a derivação que ``esquece'' $X$:

	$$
		\dernote{\rules}{}{S'\pars{\aprs{a,X},\aprs{T\{\dual{a}\},Y}}}
		{\leaf{S'\aprs{\pars{T\{\dual{a}\},\aprs{a,X}},Y}}}
	$$			
	
	Isto se $\occ{X} \cap \occ{Y} = \emptyset$. Mas se $\occ{X} \cap \occ{Y} \neq \emptyset$ a estrutura já não seria provável pela condição $C_{2}$ do Teorema \ref{teorema:condicoes}.	

	O resultado segue por indução.

\item Case 3: \ \ \ $S'\pars{\aprs{R\{a\},X},\aprs{T\{\dual{a}\},Y}}$, \ \ $R\{\circ\} \neq \circ$ \ \ e \ \  $T\{\circ\} \neq \circ$


		Nesse caso há duas hipóteses, sendo que necessariamente pelo menos uma das duas ocorre:
		
		\begin{enumerate}
			\item $R\{a\} \cap Y = \emptyset$
				
				Nesse caso podemos usar o fato de que $R\{a\} \cap Y = \emptyset$, ``esquecer'' $X$ e fazer:
				
				$$
					\dernote{\rules}{}{S'\pars{\aprs{R\{a\},X},\aprs{T\{\dual{a}\},Y}}}
					{\leaf{S'\aprs{\pars{T\{\dual{a}\},\aprs{R\{a\},X}},Y}}}
				$$
				
				Isto se $\occ{X} \cap \occ{Y} = \emptyset$. Mas se $\occ{X} \cap \occ{Y} \neq \emptyset$ a estrutura já não seria provável pela condição $C_{2}$ do Teorema \ref{teorema:condicoes}.
				
				O resultado segue por indução.
				
			\item $T\{\dual{a}\} \cap X = \emptyset$
			
				Nesse caso podemos usar o fato de que $T\{\dual{a}\} \cap X = \emptyset$, ``esquecer'' $Y$ e fazer:
			
				$$
					\dernote{\rules}{}{S'\pars{\aprs{R\{a\},X},\aprs{T\{\dual{a}\},Y}}}
					{\leaf{S'\aprs{\pars{R\{a\},\aprs{T\{\dual{a}\},Y}},X}}}										
				$$
				
				Isto se $\occ{X} \cap \occ{Y} = \emptyset$. Mas se $\occ{X} \cap \occ{Y} \neq \emptyset$ a estrutura já não seria provável pela condição $C_{2}$ do Teorema \ref{teorema:condicoes}.
				
				O resultado segue por indução.
			
		\end{enumerate}
		
		Falta apenas mostrar que $R\{a\} \cap Y = \emptyset$ ou $T\{\dual{a}\} \cap X = \emptyset$ deve ocorrer. Imagine, por contradição, que $R\{a\} \cap Y \neq \emptyset$ e $T\{\dual{a}\} \cap X \neq \emptyset$. Então as seguintes asserções são verdadeiras:
		
		$\exists n \in \occ{Y}. \dual{n} \in \occ{R\{a\}} \implies 
			\left\{ 
				\begin{array}{ll}
					Y = Y'\{n\} \ \ \wedge \\
					R\{a\} = R'\{a,\dual{n}\} 
				\end{array}
			\right.		
		$
		
		$\exists m \in \occ{Y}. \dual{m} \in \occ{T\{ \dual{a} \}} \implies 
			\left\{ 
				\begin{array}{ll}
					X = X'\{m\} \ \ \wedge \\
					T\{\dual{a}\} = T'\{\dual{a},\dual{m}\} 
				\end{array}
			\right.		
		$
		
		Tomemos o caso de $R\{a\} = R'\{a,\dual{n}\}$. Há apenas duas possibilidades: 
		
		$R\{a\} = R'\{a,\dual{n}\} \implies 
			\left\{ 
				\begin{array}{ll}
					R'\{a,\dual{n}\} = R''\pars{P\{a\},P'\{\dual{n}\}} \ \ \vee \\
					R'\{a,\dual{n}\} = R''\aprs{P\{a\},P'\{\dual{n}\}}
				\end{array}
			\right.	
		$
		
		Similarmente, para $T\{\dual{a}\} = T'\{\dual{a},\dual{m}\}$ também há apenas duas possibilidades:
		
		$T\{\dual{a}\} = T'\{\dual{a},\dual{m}\} \implies 
			\left\{ 
				\begin{array}{ll}
					T'\{\dual{a},\dual{m}\} = T''\pars{Q\{\dual{a}\},Q'\{\dual{m}\}} \ \ \vee \\
					T'\{\dual{a},\dual{m}\} = T''\aprs{Q\{\dual{a}\},Q'\{\dual{m}\}}
				\end{array}
			\right.	
		$
		
		Combinando as possibilidades para $R\{a\}$ e $T\{\dual{a}\}$, há, então, quatro possibilidades a serem avaliadas:
		
		\begin{enumerate}
			\item $R'\{a,\dual{n}\} = R''\pars{P\{a\},P'\{\dual{n}\}}$ \ \ e \ \ $T'\{\dual{a},\dual{m}\} = T''\pars{Q\{\dual{a}\},Q'\{\dual{m}\}}$ \\
			
			Nesse caso $S = \pars{ \aprs{ R''\pars{P\{a\},P'\{\dual{n}\}} ,X'\{m\} }, \aprs{ T''\pars{Q\{\dual{a}\},Q'\{\dual{m}\}} , Y'\{n\} } } $.											
				
			\item $R'\{a,\dual{n}\} = R''\pars{P\{a\},P'\{\dual{n}\}}$ \ \ e \ \ $T'\{\dual{a},\dual{m}\} = T''\aprs{Q\{\dual{a}\},Q'\{\dual{m}\}}$ \\
			
			Nesse caso $S = \pars{ \aprs{ R''\pars{P\{a\},P'\{\dual{n}\}} , X'\{m\} }, \aprs{ T''\aprs{Q\{\dual{a}\},Q'\{\dual{m}\}} , Y'\{n\} } }$
			
			\item $R'\{a,\dual{n}\} = R''\aprs{P\{a\},P'\{\dual{n}\}}$ \ \ e \ \ $T'\{\dual{a},\dual{m}\} = T''\pars{Q\{\dual{a}\},Q'\{\dual{m}\}}$ \\
			
			Nesse caso $S = \pars{ \aprs{ R''\aprs{P\{a\},P'\{\dual{n}\}} , X'\{m\} }, \aprs{ T''\pars{Q\{\dual{a}\},Q'\{\dual{m}\}} , Y'\{n\} } }$
			
			\item $R'\{a,\dual{n}\} = R''\aprs{P\{a\},P'\{\dual{n}\}}$ \ \ e \ \ $T'\{\dual{a},\dual{m}\} = T''\aprs{Q\{\dual{a}\},Q'\{\dual{m}\}}$ \\
			
			Nesse caso $S = \pars{ \aprs{ R''\aprs{P\{a\},P'\{\dual{n}\}} , X'\{m\} }, \aprs{ T''\aprs{Q\{\dual{a}\},Q'\{\dual{m}\}} , Y'\{n\} } }$
				
		\end{enumerate}
		
		Em qualquer dos casos acima, temos que $S$ possui uma subestrutura da forma: 
			
			$$
				\xymatrix{
					m \ar@{-}[r] \ar@{-}[d] \ar@{~}[dr]  & n  \ar@{-}[d] \\
					\dual{m} \ar@{-}[r] \ar@{~}[ur] & \dual{n} \\
				}	
			$$
			o que, pela condição $C_{2}$ do Teorema \ref{teorema:condicoes}, mostra que a estrutura $S$ já não seria, desde o princípio, provável, o que entra em contradição com a hipótese de que $S$ é provável. Logo, não é o caso em que $R\{a\} \cap Y \neq \emptyset$ e $T\{\dual{a}\} \cap X \neq \emptyset$.

\end{itemize}

\end{proof}

\end{Lemma}

==> resumo.tex <==
A lógica é a ciência das inferências corretas, e um sistema lógico formal é uma ferramenta para demonstrar proposições em uma certa lógica de maneira correta. Há muitos sistemas lógicos formais, e muitas maneiras de formalizá-los, por exemplo, usando dedução natural ou cálculo de seqüentes. O cálculo de estruturas (\cos) é um novo formalismo proposto por Alessio Guglielmi em 2004 que generaliza o cálculo de seqüentes no sentido de que regras de inferência podem ser aplicadas em qualquer profundidade dentro de uma fórmula, em vez de apenas no conectivo principal. Com esta característica, demonstrações em \cos\ são menores do que em qualquer outro formalismo que suporte provas analíticas. Apesar de ser interessante ter esta nova liberdade e expressividade do cálculo de estruturas, sob o ponto de vista de construção de demonstrações, mais liberdade significa um espaço de busca maior. E isto deve ser restringido quando se procura pela automação completa de sistemas dedutivos. Alguns esforços foram realizados para reduzir este não determinismo, mas se tratam de abordagens basicamente operacionais, e nenhum resultado teórico sólido a respeito do comportamento computacional do \cos\ foi obtido até agora. O foco principal desta dissertação é discutir caminhos para propor uma estratégia de demonstração para \cos\ adequada à implementação. Esta estratégia deve ser teórica, e não puramente operacional. Nós introduzimos o conceito de número de incoerência de subestruturas dentro de uma estrutura e usamos este conceito para atingir nosso resultado principal: um algoritmo que, de acordo com a nossa conjectura, corresponde a uma estratégia de demonstração para toda estrutura demonstrável no subsistema \FBV\ (a lógica linear multiplicativa \MLL\ estendida pela regra \mix) contendo apenas pares de átomos distintos dois a dois. Nosso algoritmo foi implementado e acreditamos que nossa estratégia seja um bom ponto de partida para explorar os aspectos computacionais do \cos\ em sistemas mais gerais, como o próprio sistema \BV.

==> teoremaX.tex <==
\begin{Lemma}[Propriedade X]
\label{lema:X}

	Seja uma estrutura $S$ da forma $S\pars{P\aprs{X\{x\}, Y\{y\}},Q\aprs{Z\{z\}, W\{w\}}}$. Não existem  derivações $\Pi_{1}$ e $\Pi_{2}$ em \FBV\ tais que:
	
	\begin{center}
		\begin{tabular}{cc}	
			$
			\strder{\Pi_{1}}{\FBV}{S\pars{P\aprs{X\{x\}, Y\{y\}},Q\aprs{Z\{z\}, W\{w\}}}}{\leaf{S'\aprs{P'\pars{X'\{x\}, W'\{w\}},Q'\pars{Y'\{y\}, Z'\{z\}}}}}
			$
	
			&		
			
			$
			\strder{\Pi_{2}}{\FBV}{S\pars{P\aprs{X\{x\}, Y\{y\}},Q\aprs{Z\{z\}, W\{w\}}}}{\leaf{S'\aprs{P'\pars{X'\{x\}, Z'\{z\}},Q'\pars{Y'\{y\}, W'\{w\}}}}}
			$	
		\end{tabular}
	\end{center}
		
	Equivalentemente, podemos enunciar o lema como:
	
	Uma subrede de interação da forma $\textsf{w}_{0}$ não pode ser transformada em uma subrede de interação da forma $\textsf{w}_{1}$ ou em uma subrede de interação da forma $\textsf{w}_{2}$, via regras de infererência de \FBV\ durante a construção de uma prova (de baixo para cima):

	$$
		\begin{tabular}{cccccc}
		
						
			& $\textsf{w}_{0}$ &  & $\textsf{w}_{1}$ & & $\textsf{w}_{2}$ \\
			
			Partindo de
			
			&		
			
			$
				\xymatrix{
					x \ar@{-}[r] \ar@{-}[d] \ar@{~}[dr]  & w \ar@{-}[d] \\
					z \ar@{-}[r] \ar@{~}[ur] &  y \\
				}	
			$
			
			&
						
			não podemos chegar a			
						
			&
			
			$
				\xymatrix{
					x \ar@{-}[r] \ar@{~}[d] \ar@{~}[dr]  & w \ar@{~}[d] \\
					z \ar@{-}[r] \ar@{~}[ur] &  y \\
				}	
			$
			
			&
			
			nem a 
			
			&
			
			$
				\xymatrix{
					x \ar@{~}[r] \ar@{-}[d] \ar@{~}[dr]  & w \ar@{-}[d] \\
					z \ar@{~}[r] \ar@{~}[ur] &  y \\
				}	
			$
			
			
			\\				
		\end{tabular}
	$$			

\begin{proof}

	Sabemos que em \FBV\ o número de aplicações de regras de inferência sobre uma estrutura $S_{1}$, demonstrável ou não, é finito. Seja $n(S_{1}) = |\rho|$ onde $\rho \in \{\ruleodown, \ruleaidown, \rules\}$ são instâncias de regras de inferência válidas em \FBV\ tais que:
	
	$$
		\dernote{\rho}{}{S_{1}}
		{\leaf{S_{2}}}
	$$
	
	Temos que, necessariamente, $n(S_{2}) < n(S_{1})$
	
	Portanto, vamos utilizar este fato para provar o lema por indução no número de possibilidades de aplicações de regras $n(S)$. 
	
	\begin{description}
		
		\item[Casos base:]
		
				\ \\			
				\begin{enumerate}
					
					\item $P\{\circ \} = \circ$
					
						Uma possibilidade é:
					
						$$
							\dernote{}{}{S\pars{\aprs{X\{ x \}, Y\{ y \}},Q\aprs{Z\{ z \}, W\{ w \}}}}
							{\leaf{S\aprs{\pars{X\{ x \},Q\aprs{Z\{ z \},W\{ w \}}},Y\{ y \}}}}
						$$
												
						Mas, com isso, $y \uparrow z$ (o que vai contra a criação da rede $\textsf{w}_{1}$) e $y \uparrow w$ (o que vai contra a criação a rede $\textsf{w}_{2}$). Dado que uma vez que criamos uma relação $\uparrow$ de baixo para cima em uma prova ela não pode mais ser desfeita, então não poderemos criar as desejadas $\textsf{w}_{1}$ ou $\textsf{w}_{2}$.
						
						A outra possibilidade é:
						
						$$
							\dernote{}{}{S\pars{\aprs{X\{ x \}, Y\{ y \}},Q\aprs{Z\{ z \}, W\{ w \}}}}
							{\leaf{S\aprs{\pars{Y\{ y \},Q\aprs{Z\{ z \},W\{ w \}}},X\{ x \}}}}
						$$
						
						Mas, com isso, $x \uparrow w$ (o que vai contra a criação da rede $\textsf{w}_{1}$) e $x \uparrow z$ (o que vai contra a criação da rede $\textsf{w}_{2}$). Dado que uma vez que criamos uma relação $\uparrow$ de baixo para cima em uma prova ela não pode mais ser desfeita, então não poderemos criar as desejadas $\textsf{w}_{1}$ ou $\textsf{w}_{2}$.
						
					\item $Q\{\circ \} = \circ$
						
						Análogo ao caso anterior.		
						
					\item Aplica-se uma instância de $\ruleaidown$ sobre um ocorrência de átomo $x$, $y$, $z$ ou $w$ e seu respectivo dual.
					
						Neste caso o átomo em questão não figura mais na rede de interação da estrutura e, portanto, claramente as subredes $\textsf{w}_{1}$ e $\textsf{w}_{2}$ não podem ser atingidas.
					
				\end{enumerate}
		
		\item[Casos indutivos:]
		
				\ \\
				Vamos argumentar baseados na última aplicação de regra $\rho$ sobre a estrutura \\
				$S\pars{P\aprs{X\{x\}, Y\{y\}},Q\aprs{Z\{z\}, W\{w\}}}$:
				
				$$
					\dernote{\rho}{}{S\pars{P\aprs{X\{x\}, Y\{y\}},Q\aprs{Z\{z\}, W\{w\}}}}
					{\leaf{S^{*}}}				
				$$
		
				Nos concentraremos nos casos em que $\rho$ é não-trivial.
		
				\begin{enumerate}				
				
					\item $\rho = \ruleaidown$
					
						\begin{enumerate}
							
							\item O redex está em $X\{ \ \}$
								
								$$
									\dernote{\ruleaidown}{}{S\pars{P\aprs{X\{x\}, Y\{y\}},Q\aprs{Z\{z\}, W\{w\}}}}
									{\leaf{S\pars{P\aprs{X^{*}\{x\}, Y\{y\}},Q\aprs{Z\{z\}, W\{w\}}}}}
								$$
								
								Na estrutura do contractum ainda temos a subrede de interação $\textsf{w}_{0}$, porém o número de possibilidades de aplicação de regras agora é menor. Podemos, então, aplicar a hipótese de indução.
								
							\item O redex está em $Y\{ \ \}$, $Z\{ \ \}$, $W\{ \ \}$, $P\{ \ \}$, $Q\{ \ \}$ ou $S\{ \ \}$
							
							Análogos ao caso anterior.
								
						\end{enumerate}
						
					\item $\rho = \rules$	
					
						\begin{enumerate}
							
							\item O redex está em $X\{ \ \}$
								
								$$
									\dernote{\rules}{}{S\pars{P\aprs{X\{x\}, Y\{y\}},Q\aprs{Z\{z\}, W\{w\}}}}
									{\leaf{S\pars{P\aprs{X^{*}\{x\}, Y\{y\}},Q\aprs{Z\{z\}, W\{w\}}}}}
								$$
								
								Na estrutura do contractum ainda temos a subrede de interação $\textsf{w}_{0}$, porém o número de possibilidades de aplicação de regras agora é menor. Podemos, então, aplicar a hipótese de indução.
								
							\item O redex está em $Y\{ \ \}$, $Z\{ \ \}$, $W\{ \ \}$, $P\{ \ \}$, $Q\{ \ \}$ ou $S\{ \ \}$
							
							Análogos ao caso anterior.
							
							\item O redex envolve $P\aprs{X\{x\}, Y\{y\}}$ e $Q\aprs{Z\{z\}, W\{w\}}$
							
								Sabemos que $P\{ \circ \} \neq \circ \neq Q\{ \circ \}$, pois senão teríamos o caso base.
								
								Vamos analisar as possibilidades para $P\aprs{X\{x\}, Y\{y\}}$:
								
								\begin{enumerate}
									
									\item $P\aprs{X\{x\}, Y\{y\}} = \pars{\aprs{X\{x\}, Y\{y\}}, P_{1}}$
									
										Mas então a estrutura seria da forma $S\pars{\aprs{X\{x\}, Y\{y\}}, P_{1}, Q\aprs{Z\{z\}, W\{w\}}}$, que é o equivalente a um dos casos base.
									
									\item $P\aprs{X\{x\}, Y\{y\}} = \aprs{X\{x\}, Y\{y\}, P_{1}}$
									
										Mas então podemos chamar $Y''\{y\} = \aprs{Y\{y\}, P_{1}}$ e temos que a estrutura é da forma $S\pars{\aprs{X\{x\}, Y''\{y\}}, P_{1}, Q\aprs{Z\{z\}, W\{w\}}}$, que é o equivalente a um dos casos base.
									
									\item $P\aprs{X\{x\}, Y\{y\}} = \aprs{\pars{P''\aprs{X\{x\}, Y\{y\}}, P_{2}}, P_{1}}$
									
								\end{enumerate}
								
								As possibilidades para $Q\aprs{Z\{z\}, W\{w\}}$ são análogas. 
								
								Portanto, o único caso a ser analisado é o em que \\
								$P\aprs{X\{x\}, Y\{y\}} = \aprs{\pars{P''\aprs{X\{x\}, Y\{y\}}, P_{2}}, P_{1}}$ e\\
								$Q\aprs{Z\{z\}, W\{w\}} = \aprs{\pars{Q''\aprs{Z\{z\}, W\{w\}}, Q_{2}}, Q_{1}}$.\\
								Façamos $P''' = \pars{P''\aprs{X\{x\}, Y\{y\}}, P_{2}}$ e\\
								$Q''' = \pars{Q''\aprs{Z\{z\}, W\{w\}}, Q_{2}}$.
								
								As possibilidades de aplicação da regra switch sobre a estrutura copar $\aprs{P''', P_{1}}$:
								
								$$
									\dernote{\rules}{}{S\pars{\aprs{P''', P_{1}},\aprs{Q''', Q_{1}}}}
									{\leaf{S\aprs{\pars{P''', \aprs{Q''', Q_{1}}},P_{1}}}}
								$$
								
								Na estrutura do contractum ainda temos a subrede de interação $\textsf{w}_{0}$, porém o número de possibilidades de aplicação de regras agora é menor. Podemos, então, aplicar a hipótese de indução.
								
								$$
									\dernote{\rules}{}{S\pars{\aprs{P''', P_{1}},\aprs{Q''', Q_{1}}}}
									{\leaf{S\aprs{\pars{P_{1}, \aprs{Q''', Q_{1}}},P'''}}}
								$$
								
								Mas, com isso, $x \uparrow w$ e $y \uparrow z$ (o que vai contra a criação da rede $\textsf{w}_{1}$) e $x \uparrow z$ e $y \uparrow w$ (o que vai contra a criação da rede $\textsf{w}_{2}$). Dado que uma vez que criamos uma relação $\uparrow$ de baixo para cima em uma prova ela não pode mais ser desfeita, então não poderemos criar as desejadas $\textsf{w}_{1}$ ou $\textsf{w}_{2}$.
								
								As possibilidades de aplicação da regra switch sobre a estrutura copar $\aprs{Q''', Q_{1}}$ são análogas.								
								
						\end{enumerate}
					
				\end{enumerate}
		
	\end{description}
	
\end{proof}

\end{Lemma}

\begin{Theorem}
	Uma estrutura da forma $S[S'(A\{a\}, \ Q\{q\}), \ \ S''(A'\{\dual{a} \}, \ Q'\{\dual{q}\})]$ não é provável em \FBV.

\begin{proof}

	Note que a estrutura possui uma subrede de interação da forma:
	
	$$
		\xymatrix{
			a \ar@{-}[r] \ar@{-}[d] \ar@{~}[dr]  & \dual{q} \ar@{-}[d] \\
			\dual{a} \ar@{-}[r] \ar@{~}[ur] &  q \\
		}				
	$$
	
	Se a estrutura for demonstrável, então uma hora necessariamente deve haver uma aplicação de regra:
	
	$$
		\dernote{\ruleaidown}{}{S\pars{a,\dual{a}}}
		{\leaf{S\{\circ\}}}
	$$
	, onde podemos chamar $\pars{a,\dual{a}} = R$. (O caso em que desejássemos argumentar baseados em $q$ e $\dual{q}$ seria análogo.)
		
	Mas sabemos que, dada uma estrutura $S\{R\}$ e duas ocorrências de átomos $a$ em $S\{ \ \}$ e $b$ em $R$, se $a \triangleleft b$ (respectivamente, $a \triangleright b$, $a \downarrow b$, $a \uparrow b$) então $a \triangleleft c$ (respectivamente, $a \triangleright c$, $a \downarrow c$, $a \uparrow c$) para todas as ocorrências de átomos $c$ em $R$.
	
	Logo, se a estrutura for provável, em um dado ponto da demonstração $a$ e $\dual{a}$ devem manter a mesma relação estrutural com \emph{todas} as ocorrências de átomos em $S$, em particular com $q$ e com $\dual{q}$.
	
	Vamos nos concentrar na subrede de interação:
	
	$$
		\xymatrix{
			a \ar@{-}[r] \ar@{-}[d] \ar@{~}[dr]  & \dual{q} \ar@{-}[d] \\
			\dual{a} \ar@{-}[r] \ar@{~}[ur] &  q \\
		}				
	$$
	
	Como não há maneira de transformar uma relação $\uparrow$ em $\downarrow$ na construção de baixo para cima de uma prova em \FBV, só nos resta tentar transformar as relações $\downarrow$ em $\uparrow$. Em particular, temos que criar pelo menos duas relações: $a \uparrow \dual{q}$ e $\dual{a} \uparrow q$.
	
	Vamos analisar os casos. Suponha que consigamos criar $a \uparrow \dual{q}$. Pela propriedade do quadrado, em na rede de interação de uma estrutura, um quadrado não pode haver exatamente três lados representando a mesma relação estrutural: deve haver um quarto lado. Portanto, teremos um dos seguintes casos:
	
	$$
		\begin{array}{ccccc}
			
			& &
			
			
				\xymatrix{
					a \ar@{~}[r] \ar@{-}[d] \ar@{~}[dr]  & \dual{q} \ar@{-}[d] \\
					\dual{a} \ar@{-}[r] \ar@{~}[ur] &  q \\
				}				
			
			
			& & \\
			
			& &
			
			\implies
			& & \\
			
			\framebox(95,85){
				I \ \			
				\xymatrix{
					a \ar@{~}[r] \ar@{~}[d] \ar@{~}[dr]  & \dual{q} \ar@{-}[d] \\
					\dual{a} \ar@{-}[r] \ar@{~}[ur] &  q \\
				}		
			}					
			
			&
			
			\vee
			
			& 
			
			\framebox(95,85){
				II \ \ 
				\xymatrix{
					a \ar@{~}[r] \ar@{-}[d] \ar@{~}[dr]  & \dual{q} \ar@{~}[d] \\
					\dual{a} \ar@{-}[r] \ar@{~}[ur] &  q \\
				}		
			}
				
			&
			
			\vee
			
			& 
			
			\framebox(95,85){
				III \ \ 
				\xymatrix{
					a \ar@{~}[r] \ar@{-}[d] \ar@{~}[dr]  & \dual{q} \ar@{-}[d] \\
					\dual{a} \ar@{~}[r] \ar@{~}[ur] &  q \\
				}			
			}
			
			\\
			
		\end{array}
	$$
	
	Mas no caso I, a estrutura não seria demonstrável, uma vez que $a \uparrow \dual{a}$. No caso II, $q \uparrow \dual{q}$ e também a estrutura não seria demonstrável. Já o caso III implicaria que, durante a construção de uma prova:
	
	$$
		\begin{tabular}{cccc}
		
						
			& $\textsf{w}_{0}$ &  & $\textsf{w}_{1}$ \\
			
			Partindo de
			
			&		
			
			$
				\xymatrix{
					a \ar@{-}[r] \ar@{-}[d] \ar@{~}[dr]  & \dual{q} \ar@{-}[d] \\
					\dual{a} \ar@{-}[r] \ar@{~}[ur] &  q \\
				}	
			$
			
			&
						
			chegamos a			
						
			&
			
			$
				\xymatrix{
					a \ar@{~}[r] \ar@{-}[d] \ar@{~}[dr]  & \dual{q} \ar@{-}[d] \\
					\dual{a} \ar@{~}[r] \ar@{~}[ur] &  q \\
				}	
			$
			\\				
		\end{tabular}
	$$
	, o que não é possível, pelo Lema \ref{lema:X}.
	
	Por outro lado, se supusermos que conseguimos criar $\dual{a} \uparrow b$, teremos casos análogos.

\end{proof}

\end{Theorem}
